Revisiting physical parameters of the benchmark brown dwarf LHS 6343 C through a HST/WFC3 secondary eclipse observation

The LHS 6343 system consists of a resolved M-dwarf binary with an evolved, negligibly irradiated brown dwarf, LHS 6343 C, orbiting the primary star. Such brown dwarf eclipsing binaries present rare and unique opportunities to calibrate sub-stellar evolutionary and atmosphere models since mass, radius, temperature and luminosity can be directly measured. We update this brown dwarf's mass (62.6+/-2.2 MJup) and radius (0.788+/-0.043 RJup) using empirical stellar relations and a Gaia DR3 distance. We use Hubble Space Telescope/WFC3 observations of an LHS 6343 C secondary eclipse to obtain a NIR emission spectrum, which matches to a spectral type of T1.5+/-1. We combine this spectrum with existing Kepler and Spitzer/IRAC secondary eclipse photometry to perform atmospheric characterization using the ATMO-2020, Sonora-Bobcat and BT-Settl model grids. ATMO-2020 models with strong non-equilibrium chemistry yield the best fit to observations across all modelled bandpasses while predicting physical parameters consistent with Gaia-dependant analogs. BT-Settl predicts values slightly more consistent with such analogs but offers a significantly poorer fit to the WFC3 spectrum. Finally, we obtain a semi-empirical measurement of LHS 6343 C's apparent luminosity by integrating its observed and modelled spectral energy distribution. Applying knowledge of the system's distance yields a bolometric luminosity of log(Lbol/Lsun) = -4.77+/-0.03 and, applying the Stefan-Boltzmann law for the known radius, an effective temperature of 1303+/-29 K. We also use the ATMO-2020 and Sonora-Bobcat evolutionary model grids to infer an age for LHS 6343 C of 2.86 +0.40-0.33 Gyr and 3.11 +0.50-0.38 Gyr respectively.

==> LHS_6343_properties___underestimated_distance_error.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%%%   Common units   %%%
%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\lbolSUN}{{\rm L_{\odot}}}
\newcommand{\lbolSUN}{L_{\odot}}
\newcommand{\massSUN}{M_{\odot}}
\newcommand{\radiusSUN}{R_{\odot}}
\newcommand{\massJUP}{M_{\text{Jup}}}
\newcommand{\radiusJUP}{R_{\text{Jup}}}
\newcommand{\KELVIN}{{\rm K}}
\newcommand{\PARSEC}{{\rm pc}}
\newcommand{\Gyr}{{\rm Gyr}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   LHS 6343 properties  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% LHS 6343 Distance
\newcommand{\vDIST}{35.67}
\newcommand{\eDIST}{0.59}
%\newcommand{\eDIST}{0.59}
\newcommand{\uDIST}{\PARSEC}
\newcommand{\sDIST}{\vDIST\pm\eDIST\,\,\uDIST}
%%% LHS 6343 Metallicity (directly from Montet 2015)
\newcommand{\vFeH}{0.03}
\newcommand{\eFeH}{0.26}
\newcommand{\uFeH}{{\rm [Fe/H]}}
\newcommand{\sFeH}{\vFeH\pm\eFeH\,\,\uFeH}
%%% LHS 6343 Metal Content (directly from Montet 2015)
\newcommand{\vMETCON}{0.02}
\newcommand{\eMETCON}{0.19}
\newcommand{\uMETCON}{{\rm [a/H]}}
\newcommand{\sMETCON}{\vMETCON\pm\eMETCON\,\,\uMETCON}

%%% LHS 6343 A+B Kepler apparent magnitude (directly from Johnson 2011)
\newcommand{\vKp}{13.104}
\newcommand{\eKp}{0.04}
\newcommand{\nKp}{$\textit{K}_{\hspace{0.01cm}P\hspace{0.02cm},\hspace{0.07cm}A+B}$}
\newcommand{\sKp}{\vKp\pm\eKp}
%%% LHS 6343 B-A Kepler relative magnitude (directly from Montet 2015)
\newcommand{\vKpBA}{0.84}
\newcommand{\eKpBA}{0.12}
\newcommand{\nKpBA}{$\Delta\textit{K}_{\hspace{0.04cm}P\hspace{0.02cm},\hspace{0.07cm}B-A}$}
\newcommand{\sKpBA}{\vKpBA\pm\eKpBA}
%%% LHS 6343 A+B 2MASS-K apparent magnitude (directly from Johnson 2011)
\newcommand{\vKs}{8.695}
\newcommand{\eKs}{0.011}
\newcommand{\nKs}{$\textit{K}_{\hspace{0.01cm}S\hspace{0.02cm},\hspace{0.07cm}A+B}$}
\newcommand{\sKs}{\vKs\pm\eKs}
%%% LHS 6343 B-A 2MASS-K relative magnitude (directly from Johnson 2011)
\newcommand{\vKsBA}{0.45}
\newcommand{\eKsBA}{0.06}
\newcommand{\nKsBA}{$\Delta\textit{K}_{\hspace{0.04cm}S\hspace{0.02cm},\hspace{0.07cm}B-A}$}
\newcommand{\sKsBA}{\vKsBA\pm\eKsBA}

%%% LHS 6343 A Mass
\newcommand{\vMASSa}{0.363} % 0.4015 with Benedict 2016
\newcommand{\eMASSa}{0.0125} % 0.018 with Benedict 2016
\newcommand{\uMASSa}{\massSUN}
\newcommand{\sMASSa}{\vMASSa\pm\eMASSa\,\,\uMASSa}
%%% LHS 6343 A Radius
\newcommand{\vRADa}{0.375}
\newcommand{\eRADa}{0.014}
\newcommand{\uRADa}{\radiusSUN}
\newcommand{\sRADa}{\vRADa\pm\eRADa\,\,\uRADa}
%%% LHS 6343 A Teff
\newcommand{\vTEFFa}{3432}
\newcommand{\eTEFFa}{108}
\newcommand{\uTEFFa}{\KELVIN}
\newcommand{\nTEFFa}{T_{\text{eff}\hspace{0.03cm},\hspace{0.07cm}A}}
\newcommand{\sTEFFa}{\vTEFFa\pm\eTEFFa\,\,\uTEFFa}
%%% LHS 6343 B Mass
\newcommand{\vMASSb}{0.297} % 0.319 with Benedict 2016
\newcommand{\eMASSb}{0.014} % 0.021 with Benedict 2016
\newcommand{\uMASSb}{\massSUN}
\newcommand{\sMASSb}{\vMASSb\pm\eMASSb\,\,\uMASSb}
%%% LHS 6343 B Radius
\newcommand{\vRADb}{0.318}
\newcommand{\eRADb}{0.014}
\newcommand{\uRADb}{\radiusSUN}
\newcommand{\sRADb}{\vRADb\pm\eRADb\,\,\uRADb}
%%% LHS 6343 B Teff
\newcommand{\vTEFFb}{3329}
\newcommand{\eTEFFb}{94}
\newcommand{\uTEFFb}{\KELVIN}
\newcommand{\nTEFFb}{T_{\text{eff}\hspace{0.03cm},\hspace{0.07cm}B}}
\newcommand{\sTEFFb}{\vTEFFb\pm\eTEFFb\,\,\uTEFFb}



%%% LHS 6343 C Mass
\newcommand{\vMASSc}{62.64} % 66.77 with Benedict 2016
\newcommand{\eMASSc}{1.37}  % 1.93 with Benedict 2016
\newcommand{\uMASSc}{\massJUP}
\newcommand{\sMASSc}{\vMASSc\pm\eMASSc\,\,\uMASSc}
%%% LHS 6343 C Radius
\newcommand{\vRADc}{0.788}
\newcommand{\eRADc}{0.032}
\newcommand{\uRADc}{\radiusJUP}
\newcommand{\sRADc}{\vRADc\pm\eRADc\,\,\uRADc}
%%% LHS 6343 C Teff
\newcommand{\vTEFFc}{1305} %1300
\newcommand{\eTEFFc}{20}   %17
\newcommand{\uTEFFc}{\KELVIN}
\newcommand{\nTEFFc}{T_{\text{eff}\hspace{0.03cm},\hspace{0.07cm}C}}
\newcommand{\sTEFFc}{\vTEFFc\pm\eTEFFc\,\,\uTEFFc}
%%% LHS 6343 C Lbol
\newcommand{\vLBOLc}{-4.77} %-4.767 %-4.773
\newcommand{\eLBOLc}{0.02}  %0.019  %0.018
\newcommand{\uLBOLc}{\text{log}(\lbolSUN)}
\newcommand{\sLBOLc}{\vLBOLc\pm\eLBOLc\,\,\uLBOLc}
%%% LHS 6343 C age (ATMO-2020)
\newcommand{\vAGEc}{2.86}  %3.71 with Benedict 2016
\newcommand{\eAGEc}{\text{}_{-0.21}^{+0.23}}  %-0.45+0.63 with Benedict 2016
\newcommand{\uAGEc}{\Gyr}
\newcommand{\sAGEc}{\vAGEc\hspace{0.08cm}\eAGEc\,\,\uAGEc}

%%% LHS 6343 C blackbody radiance emittance
\newcommand{\vBBRc}{1.64}  %1.6206
\newcommand{\eBBRc}{0.10}  %0.0857
\newcommand{\uBBRc}{{\rm erg~s^{-1}~cm^{-2}}}
\newcommand{\sBBRc}{(\vBBRc\pm\eBBRc)\hspace{0.1cm}\times10^8\,\,\uBBRc}
%%% LHS 6343 C age (Sonora-Bobcat)
\newcommand{\vAGEcSB}{3.11}  %4.19 with Benedict 2016
\newcommand{\eAGEcSB}{\text{}_{-0.25}^{+0.30}} %-0.58+0.92 with Benedict 2016
\newcommand{\uAGEcSB}{\Gyr}
\newcommand{\sAGEcSB}{\vAGEcSB\hspace{0.08cm}\eAGEcSB\,\,\uAGEcSB}
%%% LHS 6343 C spectral type
\newcommand{\vSPTc}{T1.5}
\newcommand{\eSPTc}{1}
\newcommand{\sSPTc}{\text{\vSPTc}\pm\text{\eSPTc}}
%%% LHS 6343 C MKO J absolute magnitude
\newcommand{\vKsC}{14.871}
\newcommand{\eKsC}{0.044}
\newcommand{\nKsC}{$M_J$}
\newcommand{\sKsC}{\vKsC\pm\eKsC}
%%% LHS 6343 C mean density
\newcommand{\vRHOc}{160}
\newcommand{\eRHOc}{19}
\newcommand{\uRHOc}{{\rm g~cm^{-3}}}
\newcommand{\sRHOc}{\vRHOc\pm\eRHOc\,\,\uRHOc}
%%% LHS 6343 C surface gravity
\newcommand{\vLOGGc}{5.399}
\newcommand{\eLOGGc}{0.033}
\newcommand{\uLOGGc}{{\rm \text{log}(cm/s^2)}}
\newcommand{\sLOGGc}{\vLOGGc\pm\eLOGGc\,\,\uLOGGc}
%%% LHS 6343 C scale factor (r/d)^2
\newcommand{\vSCALc}{2.62}
\newcommand{\eSCALc}{0.20}
\newcommand{\sSCALc}{(\vSCALc\pm\eSCALc)\times10^{-21}}
%%% LHS 6343 C semimajor axis
\newcommand{\vSMAc}{0.08}
\newcommand{\eSMAc}{0.003}
\newcommand{\uSMAc}{{\rm AU}}
\newcommand{\sSMAc}{\vSMAc\pm\eSMAc\,\,\uSMAc}
%%% LHS 6343 C equilibrium temperature
\newcommand{\vTEQc}{358}
\newcommand{\eTEQc}{11}
\newcommand{\uTEQc}{\KELVIN}
\newcommand{\sTEQc}{\vTEQc\pm\eTEQc\,\,\uTEQc}


